Multilingual Prompt Localization for Agent-as-a-Judge: Language and Backbone Sensitivity in Requirement-Level Evaluation

Evaluation language is typically treated as a fixed English default in agentic code benchmarks, yet we show that changing the judge's language can invert backbone rankings. We localize the Agent-as-a-Judge prompt stack to five typologically diverse languages (English, Arabic, Turkish, Chinese, Hindi) and evaluate 55 DevAI development tasks across three developer-agent frameworks and six judge backbones, totaling 4950 judge runs. The central finding is that backbone and language interact: GPT-4o achieves the highest satisfaction in English (44.72\%), while Gemini leads in Arabic (51.72\%, $p<0.001$ vs.\ GPT-4o) and Hindi (53.22\%). No single backbone dominates across all languages, and inter-backbone agreement on individual requirement judgments is modest (Fleiss' $\kappa \leq 0.231$). A controlled ablation further shows that localizing judge-side instructions, not just benchmark content, can be decisive: Hindi satisfaction drops from 42.8\% to 23.2\% under partial localization. These results indicate that language should be treated as an explicit evaluation variable in agentic benchmarks. Full requirement-level judgments and runtime statistics are released for reproducibility.

==> fig1_tikz.tex <==
\begin{figure*}[t]
\centering
\begin{tikzpicture}
  \node[font=\small\bfseries, anchor=south] at (4.125, 3.15) {Mean Task-Level Satisfaction (\%)};
  \node[anchor=east, font=\tiny] at (1.42,2.75) {GPT-4o};
  \fill[fill={rgb,255:red,26,96,162}] (1.500,2.500) rectangle (2.550,3.000);
  \node[font=\tiny\bfseries, text=white] at (2.025,2.750) {44.7};
  \fill[fill={rgb,255:red,115,178,216}] (2.550,2.500) rectangle (3.600,3.000);
  \node[font=\tiny\bfseries, text=black] at (3.075,2.750) {26.2};
  \fill[fill={rgb,255:red,36,116,182}] (3.600,2.500) rectangle (4.650,3.000);
  \node[font=\tiny\bfseries, text=white] at (4.125,2.750) {40.5};
  \fill[fill={rgb,255:red,32,111,179}] (4.650,2.500) rectangle (5.700,3.000);
  \node[font=\tiny\bfseries, text=white] at (5.175,2.750) {41.5};
  \fill[fill={rgb,255:red,27,99,166}] (5.700,2.500) rectangle (6.750,3.000);
  \node[font=\tiny\bfseries, text=white] at (6.225,2.750) {44.0};
  \node[anchor=east, font=\tiny] at (1.42,2.25) {GPT-5.4};
  \fill[fill={rgb,255:red,214,229,244}] (1.500,2.000) rectangle (2.550,2.500);
  \node[font=\tiny\bfseries, text=black] at (2.025,2.250) {9.1};
  \fill[fill={rgb,255:red,167,203,230}] (2.550,2.000) rectangle (3.600,2.500);
  \node[font=\tiny\bfseries, text=black] at (3.075,2.250) {18.4};
  \fill[fill={rgb,255:red,152,196,226}] (3.600,2.000) rectangle (4.650,2.500);
  \node[font=\tiny\bfseries, text=black] at (4.125,2.250) {20.7};
  \fill[fill={rgb,255:red,214,229,244}] (4.650,2.000) rectangle (5.700,2.500);
  \node[font=\tiny\bfseries, text=black] at (5.175,2.250) {9.1};
  \fill[fill={rgb,255:red,134,187,221}] (5.700,2.000) rectangle (6.750,2.500);
  \node[font=\tiny\bfseries, text=black] at (6.225,2.250) {23.3};
  \node[anchor=east, font=\tiny] at (1.42,1.75) {Sonnet 4.6};
  \fill[fill={rgb,255:red,171,206,231}] (1.500,1.500) rectangle (2.550,2.000);
  \node[font=\tiny\bfseries, text=black] at (2.025,1.750) {17.7};
  \fill[fill={rgb,255:red,192,216,237}] (2.550,1.500) rectangle (3.600,2.000);
  \node[font=\tiny\bfseries, text=black] at (3.075,1.750) {14.5};
  \fill[fill={rgb,255:red,183,211,234}] (3.600,1.500) rectangle (4.650,2.000);
  \node[font=\tiny\bfseries, text=black] at (4.125,1.750) {16.0};
  \fill[fill={rgb,255:red,200,220,239}] (4.650,1.500) rectangle (5.700,2.000);
  \node[font=\tiny\bfseries, text=black] at (5.175,1.750) {13.1};
  \fill[fill={rgb,255:red,199,220,239}] (5.700,1.500) rectangle (6.750,2.000);
  \node[font=\tiny\bfseries, text=black] at (6.225,1.750) {13.3};
  \node[anchor=east, font=\tiny] at (1.42,1.25) {Gemini 3 Flash};
  \fill[fill={rgb,255:red,65,139,195}] (1.500,1.000) rectangle (2.550,1.500);
  \node[font=\tiny\bfseries, text=white] at (2.025,1.250) {35.2};
  \fill[fill={rgb,255:red,13,63,124}] (2.550,1.000) rectangle (3.600,1.500);
  \node[font=\tiny\bfseries, text=white] at (3.075,1.250) {51.7};
  \fill[fill={rgb,255:red,38,117,183}] (3.600,1.000) rectangle (4.650,1.500);
  \node[font=\tiny\bfseries, text=white] at (4.125,1.250) {40.3};
  \fill[fill={rgb,255:red,57,133,191}] (4.650,1.000) rectangle (5.700,1.500);
  \node[font=\tiny\bfseries, text=white] at (5.175,1.250) {36.7};
  \fill[fill={rgb,255:red,11,56,116}] (5.700,1.000) rectangle (6.750,1.500);
  \node[font=\tiny\bfseries, text=white] at (6.225,1.250) {53.2};
  \node[anchor=east, font=\tiny] at (1.42,0.75) {DeepSeek V3.2};
  \fill[fill={rgb,255:red,203,222,240}] (1.500,0.500) rectangle (2.550,1.000);
  \node[font=\tiny\bfseries, text=black] at (2.025,0.750) {12.3};
  \fill[fill={rgb,255:red,225,236,247}] (2.550,0.500) rectangle (3.600,1.000);
  \node[font=\tiny\bfseries, text=black] at (3.075,0.750) {6.0};
  \fill[fill={rgb,255:red,199,219,239}] (3.600,0.500) rectangle (4.650,1.000);
  \node[font=\tiny\bfseries, text=black] at (4.125,0.750) {13.3};
  \fill[fill={rgb,255:red,195,217,238}] (4.650,0.500) rectangle (5.700,1.000);
  \node[font=\tiny\bfseries, text=black] at (5.175,0.750) {14.1};
  \fill[fill={rgb,255:red,171,205,231}] (5.700,0.500) rectangle (6.750,1.000);
  \node[font=\tiny\bfseries, text=black] at (6.225,0.750) {17.8};
  \node[anchor=east, font=\tiny] at (1.42,0.25) {Qwen3.5-9B};
  \fill[fill={rgb,255:red,235,243,251}] (1.500,0.000) rectangle (2.550,0.500);
  \node[font=\tiny\bfseries, text=black] at (2.025,0.250) {3.2};
  \fill[fill={rgb,255:red,231,240,249}] (2.550,0.000) rectangle (3.600,0.500);
  \node[font=\tiny\bfseries, text=black] at (3.075,0.250) {4.3};
  \fill[fill={rgb,255:red,232,241,250}] (3.600,0.000) rectangle (4.650,0.500);
  \node[font=\tiny\bfseries, text=black] at (4.125,0.250) {4.0};
  \fill[fill={rgb,255:red,233,242,250}] (4.650,0.000) rectangle (5.700,0.500);
  \node[font=\tiny\bfseries, text=black] at (5.175,0.250) {3.7};
  \fill[fill={rgb,255:red,232,241,250}] (5.700,0.000) rectangle (6.750,0.500);
  \node[font=\tiny\bfseries, text=black] at (6.225,0.250) {4.1};
  \node[font=\tiny, anchor=north] at (2.025,-0.08) {EN};
  \node[font=\tiny, anchor=north] at (3.075,-0.08) {AR};
  \node[font=\tiny, anchor=north] at (4.125,-0.08) {TR};
  \node[font=\tiny, anchor=north] at (5.175,-0.08) {ZH};
  \node[font=\tiny, anchor=north] at (6.225,-0.08) {HI};
  \draw[white, line width=0.6pt] (1.5,0.000) -- (6.75,0.000);
  \draw[white, line width=0.6pt] (1.5,0.500) -- (6.75,0.500);
  \draw[white, line width=0.6pt] (1.5,1.000) -- (6.75,1.000);
  \draw[white, line width=0.6pt] (1.5,1.500) -- (6.75,1.500);
  \draw[white, line width=0.6pt] (1.5,2.000) -- (6.75,2.000);
  \draw[white, line width=0.6pt] (1.5,2.500) -- (6.75,2.500);
  \draw[white, line width=0.6pt] (1.5,3.000) -- (6.75,3.000);
  \draw[white, line width=0.6pt] (1.500,0) -- (1.500,3.0);
  \draw[white, line width=0.6pt] (2.550,0) -- (2.550,3.0);
  \draw[white, line width=0.6pt] (3.600,0) -- (3.600,3.0);
  \draw[white, line width=0.6pt] (4.650,0) -- (4.650,3.0);
  \draw[white, line width=0.6pt] (5.700,0) -- (5.700,3.0);
  \draw[white, line width=0.6pt] (6.750,0) -- (6.750,3.0);
  \node[font=\small\bfseries, anchor=south] at (11.175, 3.15) {Task Solve Rate (\%)};
  \node[anchor=east, font=\tiny] at (8.47,2.75) {GPT-4o};
  \fill[fill={rgb,255:red,253,173,109}] (8.550,2.500) rectangle (9.600,3.000);
  \node[font=\tiny\bfseries, text=black] at (9.075,2.750) {3.0};
  \fill[fill={rgb,255:red,253,193,140}] (9.600,2.500) rectangle (10.650,3.000);
  \node[font=\tiny\bfseries, text=black] at (10.125,2.750) {2.4};
  \fill[fill={rgb,255:red,253,211,168}] (10.650,2.500) rectangle (11.700,3.000);
  \node[font=\tiny\bfseries, text=black] at (11.175,2.750) {1.8};
  \fill[fill={rgb,255:red,253,211,168}] (11.700,2.500) rectangle (12.750,3.000);
  \node[font=\tiny\bfseries, text=black] at (12.225,2.750) {1.8};
  \fill[fill={rgb,255:red,253,193,140}] (12.750,2.500) rectangle (13.800,3.000);
  \node[font=\tiny\bfseries, text=black] at (13.275,2.750) {2.4};
  \node[anchor=east, font=\tiny] at (8.47,2.25) {GPT-5.4};
  \fill[fill={rgb,255:red,253,222,190}] (8.550,2.000) rectangle (9.600,2.500);
  \node[font=\tiny\bfseries, text=black] at (9.075,2.250) {1.2};
  \fill[fill={rgb,255:red,254,233,212}] (9.600,2.000) rectangle (10.650,2.500);
  \node[font=\tiny\bfseries, text=black] at (10.125,2.250) {0.6};
  \fill[fill={rgb,255:red,254,233,212}] (10.650,2.000) rectangle (11.700,2.500);
  \node[font=\tiny\bfseries, text=black] at (11.175,2.250) {0.6};
  \fill[fill={rgb,255:red,254,233,212}] (11.700,2.000) rectangle (12.750,2.500);
  \node[font=\tiny\bfseries, text=black] at (12.225,2.250) {0.6};
  \fill[fill={rgb,255:red,255,245,235}] (12.750,2.000) rectangle (13.800,2.500);
  \node[font=\tiny\bfseries, text=black] at (13.275,2.250) {0.0};
  \node[anchor=east, font=\tiny] at (8.47,1.75) {Sonnet 4.6};
  \fill[fill={rgb,255:red,255,245,235}] (8.550,1.500) rectangle (9.600,2.000);
  \node[font=\tiny\bfseries, text=black] at (9.075,1.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (9.600,1.500) rectangle (10.650,2.000);
  \node[font=\tiny\bfseries, text=black] at (10.125,1.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (10.650,1.500) rectangle (11.700,2.000);
  \node[font=\tiny\bfseries, text=black] at (11.175,1.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (11.700,1.500) rectangle (12.750,2.000);
  \node[font=\tiny\bfseries, text=black] at (12.225,1.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (12.750,1.500) rectangle (13.800,2.000);
  \node[font=\tiny\bfseries, text=black] at (13.275,1.750) {0.0};
  \node[anchor=east, font=\tiny] at (8.47,1.25) {Gemini 3 Flash};
  \fill[fill={rgb,255:red,250,134,54}] (8.550,1.000) rectangle (9.600,1.500);
  \node[font=\tiny\bfseries, text=black] at (9.075,1.250) {4.2};
  \fill[fill={rgb,255:red,208,74,9}] (9.600,1.000) rectangle (10.650,1.500);
  \node[font=\tiny\bfseries, text=white] at (10.125,1.250) {6.7};
  \fill[fill={rgb,255:red,243,117,40}] (10.650,1.000) rectangle (11.700,1.500);
  \node[font=\tiny\bfseries, text=white] at (11.175,1.250) {4.8};
  \fill[fill={rgb,255:red,253,193,140}] (11.700,1.000) rectangle (12.750,1.500);
  \node[font=\tiny\bfseries, text=black] at (12.225,1.250) {2.4};
  \fill[fill={rgb,255:red,236,100,25}] (12.750,1.000) rectangle (13.800,1.500);
  \node[font=\tiny\bfseries, text=white] at (13.275,1.250) {5.5};
  \node[anchor=east, font=\tiny] at (8.47,0.75) {DeepSeek V3.2};
  \fill[fill={rgb,255:red,255,245,235}] (8.550,0.500) rectangle (9.600,1.000);
  \node[font=\tiny\bfseries, text=black] at (9.075,0.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (9.600,0.500) rectangle (10.650,1.000);
  \node[font=\tiny\bfseries, text=black] at (10.125,0.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (10.650,0.500) rectangle (11.700,1.000);
  \node[font=\tiny\bfseries, text=black] at (11.175,0.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (11.700,0.500) rectangle (12.750,1.000);
  \node[font=\tiny\bfseries, text=black] at (12.225,0.750) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (12.750,0.500) rectangle (13.800,1.000);
  \node[font=\tiny\bfseries, text=black] at (13.275,0.750) {0.0};
  \node[anchor=east, font=\tiny] at (8.47,0.25) {Qwen3.5-9B};
  \fill[fill={rgb,255:red,255,245,235}] (8.550,0.000) rectangle (9.600,0.500);
  \node[font=\tiny\bfseries, text=black] at (9.075,0.250) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (9.600,0.000) rectangle (10.650,0.500);
  \node[font=\tiny\bfseries, text=black] at (10.125,0.250) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (10.650,0.000) rectangle (11.700,0.500);
  \node[font=\tiny\bfseries, text=black] at (11.175,0.250) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (11.700,0.000) rectangle (12.750,0.500);
  \node[font=\tiny\bfseries, text=black] at (12.225,0.250) {0.0};
  \fill[fill={rgb,255:red,255,245,235}] (12.750,0.000) rectangle (13.800,0.500);
  \node[font=\tiny\bfseries, text=black] at (13.275,0.250) {0.0};
  \node[font=\tiny, anchor=north] at (9.075,-0.08) {EN};
  \node[font=\tiny, anchor=north] at (10.125,-0.08) {AR};
  \node[font=\tiny, anchor=north] at (11.175,-0.08) {TR};
  \node[font=\tiny, anchor=north] at (12.225,-0.08) {ZH};
  \node[font=\tiny, anchor=north] at (13.275,-0.08) {HI};
  \draw[white, line width=0.6pt] (8.55,0.000) -- (13.8,0.000);
  \draw[white, line width=0.6pt] (8.55,0.500) -- (13.8,0.500);
  \draw[white, line width=0.6pt] (8.55,1.000) -- (13.8,1.000);
  \draw[white, line width=0.6pt] (8.55,1.500) -- (13.8,1.500);
  \draw[white, line width=0.6pt] (8.55,2.000) -- (13.8,2.000);
  \draw[white, line width=0.6pt] (8.55,2.500) -- (13.8,2.500);
  \draw[white, line width=0.6pt] (8.55,3.000) -- (13.8,3.000);
  \draw[white, line width=0.6pt] (8.550,0) -- (8.550,3.0);
  \draw[white, line width=0.6pt] (9.600,0) -- (9.600,3.0);
  \draw[white, line width=0.6pt] (10.650,0) -- (10.650,3.0);
  \draw[white, line width=0.6pt] (11.700,0) -- (11.700,3.0);
  \draw[white, line width=0.6pt] (12.750,0) -- (12.750,3.0);
  \draw[white, line width=0.6pt] (13.800,0) -- (13.800,3.0);
\end{tikzpicture}
\caption{Backbone-by-language heatmaps averaged over three developer-agent frameworks. \textbf{Left:} Mean task-level requirement satisfaction. \textbf{Right:} Task Solve Rate. The strongest backbone varies across languages: GPT-4o leads in English, while Gemini leads in Arabic and Hindi, showing that evaluation outcomes depend jointly on language and backbone.}
\label{fig:intro_backbone_language_heatmap}
\end{figure*}
